Barbed Similarity for the $\pi$-Calculus in Beluga: A Case Study in Coinductive Reasoning

We formalize strong barbed similarity for the pi-calculus in the Beluga proof assistant, completing a line of work addressing the Concurrent Calculi Formalization Benchmark. By extending previous developments to include replication, we give a coinductive encoding of behavioral equivalence based on barbs and internal actions. Using Beluga's copattern-based coinduction, we obtain concise and compositional proofs, including compatibility properties and a context lemma characterizing barbed precongruence. The case study demonstrates the effectiveness of combining HOAS and coinductive reasoning for mechanizing concurrent calculi.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{Hermant, Tourret (Eds.): International Workshop on Logical Frameworks\\and Meta-Languages, Theory and Practice (LFMTP 26)\\
EPTCS 448, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.448.1}{10.4204/EPTCS.448.1}}
\pdfoutput=1

